Distilling Self-Supervised Vision Transformers for Weakly-Supervised Few-Shot Classification & Segmentation

We address the task of weakly-supervised few-shot image classification and segmentation, by leveraging a Vision Transformer (ViT) pretrained with self-supervision. Our proposed method takes token representations from the self-supervised ViT and leverages their correlations, via self-attention, to produce classification and segmentation predictions through separate task heads. Our model is able to effectively learn to perform classification and segmentation in the absence of pixel-level labels during training, using only image-level labels. To do this it uses attention maps, created from tokens generated by the self-supervised ViT backbone, as pixel-level pseudo-labels. We also explore a practical setup with ``mixed" supervision, where a small number of training images contains ground-truth pixel-level labels and the remaining images have only image-level labels. For this mixed setup, we propose to improve the pseudo-labels using a pseudo-label enhancer that was trained using the available ground-truth pixel-level labels. Experiments on Pascal-5i and COCO-20i demonstrate significant performance gains in a variety of supervision settings, and in particular when little-to-no pixel-level labels are available.

==> sec/99_problem.tex <==
% !TEX root = ../main.tex


\section{Problem setup}
In this paper we tackle few-shot classification and segmentation~\cite{ifsl}. 
Given a few-labeled support images for target classes, a few-shot learner i) identifies the presence of the each target class in a query image and ii) semantically segment it out.
% In this problem setup, we are given a few-labeled support images for target classes;
Specifically, a given few-shot labeled support set contains $K$ labeled instances for each $N$ target classes
% $\mathcal{C}_\texts$ , such as $\mathcal{S}=\{ (\bx_\texts^{(i)}, y_\texts^{(i)}) | y_\texts^{(i)} \in \mathcal{C}_\texts \}^{NK}_{i=1}$
as conventionally called as an $N$-way $K$-shot episode~\cite{matchingnet, ravi2016optimization}.
Based on the few support images, the learner recognizes a query image by predicting its $N$-class presence $\hat{\by}_\textcls$ and its segmentation mask $\hat{\bY}_\textseg$.
To meta-learn such a few-shot learner, an annotated training dataset from a disjoint class set is used to simulate such few-shot learning episodes of which annotations can either be class tags
\footnote{The term ``class'' tag throughout this paper denotes a relative class membership of whether the query contains a relevant semantics with a target support class rather than a certain absolute category.}
(weak supervision) or segmentation mask annotations (strong supervision).
The annotations can be generalized such that a small portion of the images have segmentation annotations while the rest of them have class tags (mixed supervision).
Note that the terms, meta-training, meta-validation, and meta-testing, are often denoted interchangeably with training, validation, and testing in this paper.
% Here the label $y_\texts^{(i)}$ is either a class tag (weak label) or a segmentation annotation (strong label). 

% We assume the class set of the query $\mathcal{C}$ is a subset of the target class set, \ie, $\mathcal{C} \subseteq \mathcal{C}_\texts$, thus it is also possible to obtain $\by_\textcls = \varnothing$ and $\bY_\textseg = \varnothing$. 
% This naturally generalizes the existing few-shot classification~\cite{matchingnet, protonet} and few-shot segmentation~\cite{shaban2017oslsm, rakelly2018cofcn}. 
